Direct Simultaneous Speech-to-Speech Translation with Variational Monotonic Multihead Attention

We present a direct simultaneous speech-to-speech translation (Simul-S2ST) model, Furthermore, the generation of translation is independent from intermediate text representations. Our approach leverages recent progress on direct speech-to-speech translation with discrete units, in which a sequence of discrete representations, instead of continuous spectrogram features, learned in an unsupervised manner, are predicted from the model and passed directly to a vocoder for speech synthesis on-the-fly. We also introduce the variational monotonic multihead attention (V-MMA), to handle the challenge of inefficient policy learning in speech simultaneous translation. The simultaneous policy then operates on source speech features and target discrete units. We carry out empirical studies to compare cascaded and direct approach on the Fisher Spanish-English and MuST-C English-Spanish datasets. Direct simultaneous model is shown to outperform the cascaded model by achieving a better tradeoff between translation quality and latency.

==> arxiv_sections/3_methodology.tex <==
\section{Methodology}
%\subsection{Simultaneous Speech-to-Units Model}
\Cref{fig:arch} illustrate the architecture of the direct Simul-S2ST model with discrete units.
The encoder reads the speech features with downsampling,
and generates a sequence of hidden representations.
Then the simultaneous policy replaces soft-attention in offline model to connect encoder and decoder.
Because of the granularity of the encoder states,
we follow the same setup as \cite{ma2020simulmt} to use a fixed pre-decision module before applying the simultaneous policy.
The policy contains two actions: \textsc{READ} and \textsc{WRITE}.
The \textsc{READ} action indicates that the model takes another chunk of speech segment to update the encoder states, %\juan{do we mention here that we're focusing on algorithmic latency and leave emformer for future work?} while the \textsc{WRITE} action predicts the discrete units.
In this paper, we use the wait-$k$ policy introduced by~\cite{ma-etal-2019-stacl}
In this work, we're focusing on algorithmic latency and leave architectures such as emformer \cite{shi2021emformer} with more efficient computation for future work.

A vocoder will be applied to the discrete units to synthesize the final speech output.
Denote the emission rate $l$, the vocoder will be called every time $l$ units are predicted.
Note that the vocoder is not used during training time.
Because the vocoder is trained on short speech segment in a non-autoregressive manner,
as shown in the results, a small $l$ can achieve good latency without a huge sacrifice on quality.

\begin{figure}[h]
    \includegraphics[width=0.5\textwidth]{figures/simul_s2st.pdf}
    \caption{Architecture of direct Simul-S2ST model with discrete units.}
    \label{fig:arch}
\end{figure}


%\subsection{Speech-to-Units with Wait-$k$ Strategy}

It is straightforward to integrate wait-$k$ strategy into the speech-to-unit model. The decoder first waits for $k$ steps and processes the beginning of input speech. Then it takes input speech and generates target discrete units concurrently.


% \subsection{Simultaneous Policy with Supervision}

% A challenge of simultaneous translation is to learn a good policy that decides when to read more input and when to generate output.
% In this work, we propose to distill the policy knowledge from an offline model into the simultaneous model.
% The intuition is that a well-trained offline model captures the dependency between inputs and outputs.


% \noindent \textbf{Offline Policy}.
% All inputs with different lengths are provided, we could know how much input is needed for each target prediction.
% Given a trained offline model, we want to export its learned policy, i.e.,
% how much input information is needed to generate a target output.
% We provide a partial input with which the offline model predicts the likelihood of each target token in the reference translation.
% The target token is ranked among all tokens in the vocabulary based on the estimated likelihood.
% Given a rank threshold $r$, if a token has a higher ranker than $r$, it suggests that the partial input contains sufficient information for this token.
% Hence when a simultaneous model could generate the token when reading that partial input.
% As partiget token so that it can be predicted with high likelihood by the offline model.

% \noindent \textbf{Knowledge distillation}. With the policy obtained from the offline model, we want to guide simultaneous model using knowledge distillation. This is done via the supervision on the simulatanous model's attention.
% Suppose that the lengths of partial inputs sorted in an increasing order $[L_{1}, \ldots, L_{i}, \ldots]$. For the $j$-th token, an offline model ranks it above the threshold $r$ when the partial input of length $L_{i}$ is given.
% In a simultaneous model, suppose that the attention vector of the target token $j$ over the sequence of encoder states is $\boldsymbol{\alpha}_{j}=[\alpha_{j,1}, \ldots, \alpha_{j,i}, \ldots]$.

% A partial input of length $L_{i-1}$ does not provide enough information to predict token $j$ while an input of length $L_{i}$ does. This implies that the source knowledge that token $j$ relies on fall in the input segment $(L_{i-1}+1, L_{i}]$. Therefore we encouage the attention of a simultaneous model to be concentrated on this segment. Accordinly, the auxiliary loss $L_{a}$ we propose is:
% \begin{align}
% L_{a} = -\sum\limits_{k=L_{i-1}+1}^{L_{i}}\alpha_{j,k}.
% \end{align}

% The auxiliary loss is added to the training objective as complimentary to the prediction loss.

==> arxiv_sections/5_experiments.tex <==
\input{tables/fisher_waitk_results.tex}

\section{Experiments}
We conduct experiments of simultaneous speech-to-speech translation on Fisher Spanish-to-English dataset \cite{post2014fisher}.
The dataset The consists of $139k$ sentences from telephone conversations in Spanish,
the corresponding Spanish text transcriptions and their English text translation.
Same as~\cite{lee2021direct},
the target speech data is generated from a high-quality in-house TTS with a single female voice.
We follow the same training setup as \citet{lee2021direct},
except that a masked attention for wait-$k$ policy is used for training \cite{ma-etal-2019-stacl}.
As to inference, we use \cite{ma2020simuleval} to simulate the real world setup with a server-client scheme.
%When synthesizing the target speech,
%silence is inserted between segments where the system has to wait for either source speech or computation of the system.

The offline cascaded system we used as baseline consists of two components: S2T and TTS.
The S2T model is the \text{s2t\_transformer\_s} architecture provided by \textsc{FAIRSEQ} S2T for speech-to-text translation \cite{wang2020fairseq},
As for the TTS, we use a Transformer model with $6$ layers,
$4$ attention heads and dimensions of $512$ and $2048$,
and a HiFi-GAN based vocoder generating speech from the predicted mel-spectrograms \cite{kong2020hifi}.
As to the simultaneous cascaded system,
its S2T module has the same architecture as the offline S2T Transformer,
and wait-$k$ strategy is integrated to enable simultaneous speech-to-text translation.
Meanwhile, for computational efficiency,
we adapt the non-autoregressive FastSpeech 2 model \cite{fastspeech2} as the incremental TTS component.
It incrementally generates utterances word-by-word, utilizing the duration predictor for segmenting output word boundaries \cite{stephenson21_interspeech}.
It further uses a lookahead of 1 word, which is equivalent to a wait-$k$ strategy at test-time \cite{ma2019stacl,ma-etal-2020-incremental},
where $k$ is two words\footnote{Wait-$(k+1)$ is equivalent to lookahead-$k$ following the definition in \cite{ma-etal-2020-incremental}}.
When running offline inference, this cascaded system scores 38.1 BLEU on the test set.

Translation quality and efficiency are important for simultaneous translation models.
Following the evaluation of speech quality~\cite{lee2021direct},
we transcribe the generated speech with a pre-trained ASR model,
and measure the BLEU score by comparing the transcription and the reference.
To have a fair comparison with offline model, discontinuities are not considered while transcribing of real-time target speech.
The computation-aware~\cite{ma2020simulmt} version of Average Lagging (AL)~\cite{ma-etal-2019-stacl}
is used to measure the latency as previous works of simultaneous translation. %\danni{Maybe we should specify how we concatenate the chunks and what we do about the pauses}


\section{Results}
% offline models

%Both cascaded and direct S2ST models are considered in our experiments.
%We use S2U model, the state-of-the-art model in offline direction S2ST with discrete units \cite{lee2021direct}.
%Instead of generating intermediate texts as cascaded model,
%S2U model predicts discrete units which are learned by HuBERT model in an unsupervised manner from target speech \cite{hsu2021hubert}.
%It is a transformer based model built upon a speech encoder, a discrete unit decoder and a vocoder for waveform generation.
%
% simultaneous models
%Simultaneous baselines in our experiments are built with the state-of-the-art techniques.
%We have a simultaneous cascaded S2T+TTS model.
%Its S2T module has the same architecture as the offline S2T Transformer,
%and wait-$k$ strategy is integrated to enable simultaneous speech-to-text translation.
%As for the incremental TTS component, for computational efficiency,
%we adapt the non-autoregressive FastSpeech 2 model \cite{fastspeech2} for incremental inference.
%It incrementally generates utterances word-by-word, utilizing the duration predictor for segmenting output word boundaries \cite{stephenson21_interspeech}.
%It further uses a lookahead of 1 word, which is equivalent to a wait-$k$ strategy at test-time \cite{ma2019stacl,ma-etal-2020-incremental},
%where $k$ is two words\footnote{Wait-$(k+1)$ is equivalent to lookahead-$k$ following the definition in \cite{ma-etal-2020-incremental}}.
%\hongyu{@Danni: can you add descriptions for the incremental TTS model?}.



% \noindent \textbf{Baselines}. Various models are included for  empirical comparisons.
% \begin{itemize}
%     \item Offline direct s2s translation \cite{lee2021direct}.
%     \item Offline cascaded s2s translation. It is a stack of a simultaneous speech-to-text model with wait-$k$ strategy and simultaneous text-to-speech synthesis model \textcolor{blue}{citation of cascaded model}.
%     \item Simultaneous cascaded s2s model. Similar to the offline cascaded model, it consists of a simultaneous s2t model and TTS model.
% \end{itemize}
% Offline models would provide an upper bound of the translation quality. As the first work in simultaneous speech translation, we leverage different strategies such as wait-$k$ strategy and monotonic multihead attention (MMA) from simultaneous machine translation.


%\section{Fisher Results}
The full results are shown as \Cref{tab:fisher_results}.
We include offline speech-to-speech models which provide an upper bound of the translation quality.
In the offline setting, the direct S2S model falls behind the cascaded model by $2.3$ BLEU.
As for the simultaneous setting, latency is an important factor besides the translation quality. 
Comparing two models, we can find that the direct approach has higher BLEU score on the high latency setting ($>4000$ ms).
Considering the difference between offline and direct models,
the better performance for direct model on high latency shows that it has the ability to handle the compounding errors.
However, in low latency region ($<4000$ ms),
the translation quality for direct model drop significantly.
The potential reason can be in wait-$k$ policy, 
a small look-ahead of $k$ hurts the discrete units more than characters.
A direction of further work can be designing a simultaneous policy specifically for discrete units.  


==> arxiv_sections/background.tex <==
\section{Background}
\subsection{Offline Direct S2ST with Direct Units}
Recently, \citet{lee2021direct} propose a method for offline direct S2ST with discrete units.
First, unsupervised continuous representations at every 20-ms frame are learned on target speech corpus by a HuBERT model \cite{hsu2021hubert}.
Then the k-means algorithm is applied to the representations to generate $K$ cluster centroids.
For each window, found the it's closest centroids index as it's discrete label. %\juan{needs fix: utterance -> window}
Denote the discrete sequence as $\mathbf{Z} = {z_1, ...z_L}$.
Given the discrete units,
\citet{lee2021direct} build a transformer-based~\cite{vaswani2017attention} speech-to-unit (S2U) model.
In the encoder, a stack of 1D-convolutional layers serve as downsampler for the speech input.
Since the target sequence is discrete, the S2U model can be trained with cross-entropy loss.
Finally, the vocoder converts the discrete units to speech signal.
\citet{lee2021direct} introduce a modified version of the HiFi-GAN neural vocoder~\cite{kong2020hifi} for unit-to-waveform conversion

%\juan{I think wait-k should be also introduced here?}
\subsection{Wait-$k$ Policy}

Wait-$k$ \cite{ma-etal-2019-stacl} is a simple and commonly used policy for simultaneous translation.
It first waits $k$ inputs,
which can be words or characters for text inputs, and frames or fbank features for speech inputs,
to collect some contextual information,
then alternates between taking inputs and generating outputs.

% \subsection{Monotonic Multihead Attention}

% \label{sec:monotonic_attention}
% Monotonic attention models~\cite{raffel2017online,chiu2018mocha,arivazhagan-etal-2019-monotonic,ma2019monotonic} are designed for the scenario where only partial input is provided to the decoder.
% At a given time when $i-1$-th target token have been predicted and $j$-th source inputs have been consumed,
% a policy consisting in a stepwise probability $p_{i,j}$ predicts whether to generate the $i$-th target token or to read the $j+1$-th source input.
% Instead of sampling the actions from the policy,
% a closed form of the expected alignment \cite{raffel2017online} $\alpha_{i,j}$ given $p_{i,j}$
% replaces the soft-attention during training:
% \begin{equation}
%     \label{eq:monotonic_attention}
%     \begin{split}
%     \hat{\alpha}_{i,j} = p_{i,j} \left((1-p_{i,j-1})\frac{
%         \hat{\alpha}_{i,j-1}}{p_{i,j-1}} + \alpha_{i-1, j}\right)\\
%     \end{split}
% \end{equation}
% While \cite{raffel2017online} assume a hard alignment between encoder and decoder
% (only one encoder state is passed to the decoder at any time),
% \citet{chiu2018mocha} introduce monotonic chunkwise attention (MoChA),
% which enables soft attention in a chunk following the moving attention head.
% \citet{arivazhagan-etal-2019-monotonic} further extend (MoChA),
% proposed monotonic infinite lookback attention (MILk),
% in which a soft attention is computed over all the previous history.
% Given the energy $u_{i,j}$ for the $i$-th decoder state and the $j$-th encoder state,
% an expected soft attention is calculated in \autoref{eq:milk_recurent}:
% \begin{equation}
%   \label{eq:milk_recurent}
%   \hat{\beta}_{i,j} = \sum_{k=j}^{|\mathbf{X}|} \left( \frac{\hat{\alpha}_{i, k} \exp(u_{i,j})}{\sum_{l=1}^k  \exp(u_{i, l})} \right)
% \end{equation}
% where $\hat{\alpha}$ is calculated from \Cref{eq:monotonic_attention}.
% $\hat{\beta}$ instead of $\hat{\alpha}$ is then used in training.
% \citet{arivazhagan-etal-2019-monotonic} also introduce latency augmented training for latency control,
% because without regularization, the attention will reach the end of sentence at the first step to minimize the target prediction cross entropy.
% Given the expected alignment $a_{i,j}$, the expected delays of all the predictions can be calculated. A latency loss $\mathcal{C}([\hat{n}(y_1),...,\hat{n}(y_N)])$ is then added to the total loss function,
% where $\mathcal{C}$ is a latency measurement function and $\hat{n}(y_i) = \sum_{j=1}^{|\mathbf{X}|} j \alpha_{i,j}$ is the expected delay of the system.
% \citet{ma2019monotonic} further extend the monotonic attention to monotonic multihead attention (MMA) for transformer models.
% The design of MMA is to enable every attention head as individual monotonic attention.
% Further, the latency is controlled by controlling the expected average and variance of the delays of all attention heads.
% In order to adapt MMA to simultaneous speech translation task and address the granular encoder states,
% \citet{ma2020simulmt} introduce MMA to speech applications. However, the policy learning on speech is not as efficient as the text task.
